Distributed Construction of Near-Optimal Compact Routing Schemes for Planar Graphs

We consider the problem of computing compact routing tables for a (weighted) planar graph $G:= (V, E,w)$ in the PRAM, CONGEST, and the novel HYBRID communication model. We present algorithms with polylogarithmic work and communication that are almost optimal in all relevant parameters, i.e., computation time, table sizes, and stretch. All algorithms are heavily randomized, and all our bounds hold w.h.p. For a given parameter $\epsilon>0$, our scheme computes labels of size $\widetilde{O}(\epsilon^{-1})$ and is computed in $\widetilde{O}(\epsilon^{-2})$ time and $\widetilde{O}(n)$ work in the PRAM and the HYBRID model and $\widetilde{O}(\epsilon^{-2} \cdot HD)$ (Here, $HD$ denotes the network's hop-diameter) time in CONGEST. The stretch of the resulting routing scheme is $1+\epsilon$. To achieve these results, we extend the divide-and-conquer framework of Li and Parter [STOC '19] and combine it with state-of-the-art distributed distance approximation algorithms [STOC '22]. Furthermore, we provide a distributed decomposition scheme, which may be of independent interest.

==> Distributed Construction of Near-Optimal Compact Routing Schemes for Planar Graphs/Sections/Dump/ClusteringToCovering.tex <==
Now suppose  that we have black-boc access to a padded decomposition algorithm \textsc{Decomp}(d) that runs in time $T_{DC}$.
This provides us a straightforward construction of a $(e^{\frac{\tau}{k}}\log^2(n),O(k))$-nice clustering in $O(e^{\frac{\tau}{k}}\log^2(n))$
given that graph's diameter is polynomial in $n$.
To this end, let $D \in O(n^c)$ be the graph's diameter and define $\Delta_i = 2^i$ for every $i=1, \dots, \log(D)$.
Note that our assumption ensures that it holds $i < c\log(n)$ and therefore $i$ is logarithmic in $n$.

\begin{algo}
\textbf{\underline{\texttt{CreateNiceClustering}}}($G$)
\begin{enumerate}
    \item Let $\mathfrak{C} = \emptyset$ be an empty clustering.
    \item For each $i \in [1,\log(D)]$ do the following:
    \begin{enumerate}
        \item Create $\tau_k$ padded decompositions with distance parameter $\Delta_i$. 
        \item Denote the resulting decompositions as $\mathcal{C}^i := \{C^{(i)}_1, \dots, C^{(i)}_{\tau_k}\}$, s.t., it holds:
        \begin{align}
            C^{(i)} := \textsc{Decomp}(G,\Delta_i)
        \end{align}
        \item Add all clusters from $\mathcal{C}^i$ to $\mathfrak{C}$.
    \end{enumerate}
    \item Return $\mathfrak{C}$  
\end{enumerate}    
\end{algo}

Since each $v$ is in exactly one cluster per decomposition, the total number of clusters that contain $v$ is $\alpha\log(n)\log(D)$.
Further, for any pair of nodes $s,t \in V$ with distance $d(s,t)$ there is cluster with a diameter $O(d(s,t))$ that contains both $s$ and $t$.
Then, we can use the center of this cluster as a \emph{routing beacon} for $s$ and $t$.

By that, we mean that our routing scheme picks a path $P_{svt} := (s \to v \to t)$ approximates the path $P_{st} = (s \to t)$.

==> Distributed Construction of Near-Optimal Compact Routing Schemes for Planar Graphs/Sections/Dump/OldProof.tex <==
\begin{appendixproof}

Let us introduce some more notation and properties before proving this Lemma.
Define the following events:
\begin{alignat*}{2}
\calC_i &= \{B_z\cap K_i\notin\{\emptyset,B_z\}\} & \qquad &
\text{``$B_z$ cut in round $i$ (by $A_i$)''}, \\
\calF_i &= \{B_z\cap K_i=\emptyset\} & & \text{``$i$ was a \texttt{no-op}
  round''}, \\
\calE_i &= \bigg\{\calC_i\wedge\bigwedge_{j<i}\calF_j\bigg\} & &
\text{``$B_z$ first cut in round $i$''.}
\end{alignat*}

Denote by $\calF_{(< i)}$ the event $\bigwedge_{j<i}\calF_j$, so that $\calE_i =
(\calC_i \land \calF_{(<i)})$.
Denote by $\calFbar_i$ the complement of $\calF_i$. Observe that $\calC_i$ (respectively $\calFbar_i$) implies that $A_i\in\calI_z$, so
\begin{eqnarray}\label{eq:full1}
\Pr[\calC_i]=\Pr[\calC_i\wedge A_i\in\calI_z]=\Pr[A_i\in\calI_z]\cdot\Pr[\calC_i\mid A_i\in\calI_z]~,\\\label{eq:full2}
\Pr[\calFbar_i]=\Pr[A_i\in\calI_z]\cdot\Pr[\calFbar_i\mid A_i\in\calI_z]~.
\end{eqnarray}
and the same holds also when conditioning on any other event. We have the following claim:

\begin{claim}\label{claim:cut}
For each $i\in N$,
\[
\Pr[\calC_i\mid \calF_{(<i)}, A_i\in\calI_z]\le (1-\delta)\cdot\left(\Pr[\calFbar_i\mid \calF_{(<i)},A_i\in \calI_z]+\frac{1}{e^b-1}\right)~.
\]
\end{claim}
\begin{proof}
Fix any graph $G_i$ and any set $A_i\subseteq V(G_i)$ that agree with the conditioning on $\calF_0,\dots \calF_{i-1}$ and so that $A_i\in \calI_z$. Denote by $\rho=d_{G_i}(A_i,B_z)$, $\bar{b}=b/(u-l)$, and let $m=\max\{l,\rho\}$ . Recall that $R_i$ is chosen independently, so
\begin{eqnarray*}
\Pr[\calFbar_i\mid \calF_0,\dots,\calF_{i-1},A_i\in \calI_z,A_i]&=&\int_m^u\frac{\bar{b} e^{-\bar{b}y}}{e^{-\bar{b}l}-e^{-\bar{b}u}}dy\\
&=&\frac{e^{-\bar{b}m}-e^{-\bar{b}u}}{e^{-\bar{b}l}-e^{-\bar{b}u}}~.
\end{eqnarray*}
Since $\calF_0,\dots,\calF_{i-1}$ occurred and $G_i\supseteq G_0\setminus(\cup_{j<i}K_j)$, we have that $B_z\subseteq
G_i$. Now if $R_i\ge\rho+2\gamma$ then by the triangle inequality
$B_z\subseteq K_i$, and the ball is ``saved''. This bounds the cut
probability thus:
\begin{eqnarray*}
\Pr[\calC_i\mid \calF_{(<i)},A_i\in \calI_z,A_i]&\le&\int_m^{\rho+2\gamma}\frac{\bar{b} e^{-\bar{b}y}}{e^{-\bar{b}l}-e^{-\bar{b}u}}dy\\
&\le&\frac{e^{-\bar{b}m}-e^{-\bar{b}(m+2\gamma)}}{e^{-\bar{b}l}-e^{-\bar{b}u}}\\
&=&\frac{e^{-\bar{b}m}(1-\delta)}{e^{-\bar{b}l}-e^{-\bar{b}u}}\\
&=&(1-\delta)\cdot\Pr[\calFbar_i\mid \calF_{(<i)},A_i\in \calI_z,A_i]+(1-\delta)\frac{e^{-\bar{b}u}}{e^{-\bar{b}l}-e^{-\bar{b}u}}\\
&=& (1-\delta)\cdot\left(\Pr[\calFbar_i\mid \calF_{(<i)},A_i\in \calI_z,A_i]+\frac{1}{e^b-1}\right)~.
\end{eqnarray*}
Finally, because the bound holds for any $A_i$, it holds without
conditioning on it.
\end{proof}


\begin{proof}[Proof of \ref{lem:cut}]

Observe that for each $i\in[N]$, the events $\left\{\calFbar_i\wedge\calF_{(<i)}\right\}$ are pairwise disjoint (this is the event that $B_z$ is either cut or contained in $K_i$ for the first time),
thus by the law of total probability,
\begin{equation}\label{eq:gq}
\sum_{i\in N}\Pr\left[\calFbar_i\wedge\calF_{(<i)}\right]\le 1~.
\end{equation}
Also, by the linearity of expectation
\begin{equation}\label{eq:lin}
\tau = \sum_{i \in }\Pr[A_i\in\calI_z]~.
\end{equation}
To bound the probability of the ball being cut, we start off with the
trivial union bound:
\begin{align*}
\Pr\left[\bigcup_{i\in N}\calE_i\right]&\le \sum_i\Pr[\calE_i] = \sum_i\Pr\left[\calC_i\wedge\calF_{(<i)}\right]\\
&=\sum_i\Pr[\calC_i\mid \calF_{(<i)}] \cdot \Pr[\calF_{(<i)}] \\
&\stackrel{\eqref{eq:full1}}{=}
  \sum_i \Pr[\calC_i \mid \calF_{(<i)}, A_i\in\calI_z]
  \cdot \Pr[A_i\in\calI_z\mid \calF_{(<i)}]
  \cdot \Pr[\calF_{(<i)}] \\
&\stackrel{\text{\footnotesize \ref{claim:cut}}}{\leq}
  \sum_i (1-\delta)\left(\Pr[\calFbar_i\mid \calF_{(<i)},A_i\in\calI_z]+\frac{1}{e^b-1}\right)
  \cdot \Pr[A_i\in\calI_z\mid \calF_{(<i)}]
  \cdot \Pr[\calF_{(<i)}] \\
 &\stackrel{\eqref{eq:full2}}{=} (1-\delta)\cdot\sum_i\Pr\left[\calFbar_i\wedge\calF_{(<i)}\right]+\sum_i\Pr\left[A_i\in\calI_z\wedge\calF_{(<i)}\right]\cdot\frac{1-\delta}{e^b-1}\\
 &\stackrel{\eqref{eq:gq}}{\le}(1-\delta)+\frac{1-\delta}{e^b-1}\cdot\sum_i\Pr[A_i\in\calI_z]\\
 &\stackrel{\eqref{eq:lin}}{=}(1-\delta)\left(1+\frac{\tau}{e^b-1}\right)~.
\end{align*}
This completes the proof.
\end{proof}

\end{appendixproof}

==> Distributed Construction of Near-Optimal Compact Routing Schemes for Planar Graphs/Sections/Intro.tex <==
Efficient communication between multiple parties is an (if not \emph{the} most) integral functionality of a distributed system.
It is ensured by so-called \emph{routing schemes}, which are distributed algorithms that control the forwarding of packets from one device to another.
Given a packet with sender $s$ and a receiver $t$, a routing scheme chooses the path that the packet takes from $s$ to $t$.
Due to their practical importance and theoretical appeal, it is no wonder that there is a rich body of research dedicated to finding efficient routing schemes.
Numerous polynomial-time sequential algorithms that compute near-optimal routing schemes for a variety of performance metrics\cite{AGM05,TZ01,AM04,BLT14,raecke02,raecke08,CR20,survey09,DBLP:conf/stoc/HaeuplerR022,GH21}.
This work considers \emph{compact routing schemes} with \emph{low stretch}.
These routing schemes optimize the distance of their routing paths about some shortest path metrics. The ratio between the distances of the routing scheme's path and the optimal path is called stretch. 
Further, the scheme only stores little additional information on each node.
Finally, it assigns a short label to each node that aids in the routing.
Naturally, these routing schemes are deeply intertwined with shortest path algorithms.
For general graphs, the best we can hope for is a stretch of $2k-1$ with routing tables of size $\Tilde{O}(n^{1/k})$ due to Erdös' girth conjecture.

The existing sequential algorithms assume that a single centralized entity has access to the complete topology and all other relevant values of the network for performing the computation. This makes them infeasible for scenarios where such an entity is unavailable (perhaps due to failures), the network is prohibitively extensive, or the system's topology is frequently changing. The nodes do not have the communication capabilities to feed their connections to a central instance in time. Therefore, we are interested in the distributed computation of routing schemes. In a fully distributed model, there is no centralized entity with global knowledge, and the system nodes have to compute the paths only by exchanging small messages with other nodes.

In recent years, there have been several breakthroughs in the \emph{distributed} computation of such routing schemes in almost optimal time.
The concrete time bounds depend on the model of computation.
In the \LOCAL model that assumes unbounded message sizes, all routing schemes can be trivially computed in $\HD$ time by gathering the topology at a single node. 
Here, \HD denotes the network's hop diameter. The distributed round complexity of computing routing schemes was therefore considered in the \CONGEST model, which uses messages of (realistic) size $O(\log(n))$. The bad news for \CONGEST is that it takes $\Tilde{O}(\!\sqrt{n}+\HD)$ rounds to compute the problem \cite{DBLP:conf/stoc/LenzenP13}. In other words, size $O(\sqrt{n})$ is an additive term compared to \LOCAL.
The good news is that this was nearly matched in a series of algorithmic results \cite{DBLP:conf/stoc/LenzenP13, DBLP:conf/podc/LenzenP15, DBLP:journals/dc/LenzenPP19, DBLP:conf/podc/ElkinN16a,ElkinN18}. 
In particular, \cite{ElkinN18} gives a solution with stretch $\bigO(k)$, routing tables of size $\tilO(n^{1/k})$, routing labels of size $\tilO(k)$ that can be computed in $\bigO\big(n^{1/2 + 1/k} \!+\! \HD\big) \cdot n^{o(1)}$ rounds.
Thus, for \CONGEST, they almost match all relevant lower bounds.
However, only some networks of interest can be faithfully modeled by \CONGEST.
In a recent article, Kuhn and Schneider \cite{KS22} consider routing schemes in the so-called \HYBRID model (first presented in \cite{AHKSS20}) where each node can additionally communicate $O(\log n)$ bits with $O(\log n)$ non-neighboring nodes.
This model is motivated by the fact that many modern communication networks exhibit more than one mode of communication. For example, in many wireless ad-hoc networks, the nodes can use satellite or cellular connections to exchange a few bits with any node in the network\footnote{However, not enough so the whole network can be gathered at a single node.}.
%Kuhn and Schneider show that in $\tilO(n^{1/3})$ rounds, one can compute \textbf{exact} routing schemes with labels of size $\tilO(n^{2/3})$ bits, or constant stretch approximations with smaller labels of $\bigO(\log n)$ bits. 
Kuhn and Schneider prove that it takes $\Tilde{O}(n^{1/3})$ rounds to compute exact routing schemes with labels of size $\bigO(n^{2/3})$ on unweighted graphs and provide an algorithm that matches this. They also give \textbf{polynomial} time lower bounds $\Omega(n^{1/f(k)})$ for routing schemes with stretch $k$ on weighted graphs. Here, $f(k)$ is a function polynomial in $k$.
The previous works clearly show the (distributed) complexity of compact routing in general graphs and provide almost time-optimal algorithms for various models. Nevertheless, in both \CONGEST and \HYBRID, there is an unavoidable dependency on $\omega(polylog(n))$ in the time complexity, at least for archiving constant stretch. 
This may be too much for real-world applications.
Thus, we consider the following question: \emph{Can we find a constant stretch compact routing scheme for a non-trivial graph class in $\Tilde{O}(HD)$ time in the \CONGEST model (and $n^{o(1)}$ time in the \HYBRID model)?}

Previous attempts to resolve this question focused on well-connected chordal graphs \cite{NisseRS10} or networks embedded into a grid graph with unit edge weight\cite{CCFHKS21, coy_routing_2022,DBLP:conf/algosensors/JungKSS18,DBLP:conf/icdcn/CastenowKS20}. In this work, we extend the latter and consider compact routing schemes for \emph{all} planar graphs, i.e., all graphs drawn in the plane without two edges intersecting. This graph class is interesting for (at least) two significant reasons. First, many real-world networks (like the Internet's backbone or special wireless networks\cite{coy_routing_2022,castenow_bounding_2019}) can be modeled as planar or nearly planar graphs. Second, planar graphs have many beneficial topological properties, allowing for efficient algorithms. For example, it is long known that this class of graphs allows for compact routing schemes with arbitrarily low stretch $1+\epsilon$ and very small routing tables of size ${O}(\epsilon^{-1}\log^2 n)$ \cite{Thorup04}.

Our main contribution is a routing scheme with stretch $(1+\epsilon)$ for any $\epsilon>0$ and labels and routing tables of size $O(\epsilon^{-1}\log^5n)$ that can be implemented fast in a distributed (and also parallel) way.
In particular, our scheme can be implemented in $\Tilde{O}(\epsilon^{-3}\cdot HD)$ time in the standard \CONGEST model, $\Tilde{O}(\epsilon^{-3})$ time in the \HYBRID model, and even in $\Tilde{O}(\epsilon^{-3})$ depth by \PRAM with $\Tilde{O}(n)$ processors.
In other words, we have slightly bigger routing tables than the best sequential algorithm, but our scheme can be computed in almost optimal time in many relevant models.
Our main tools are the separator-based decomposition by Li and Parter \cite{DBLP:conf/stoc/LiP19} and the approximate shortest path algorithm by Rozhon \textcircled{r} al. \cite{DBLP:conf/stoc/RozhonGHZL22}.
Further, we present a scheme of constant stretch and tables of size $O(\log^4(n))$ that can be computed simultaneously.
Our second construction is based on (a variant of) padded decompositions for planar graphs, which may be of independent interest.
This algorithm further uses techniques from sequential decomposition algorithms for planar graphs\cite{DBLP:conf/stoc/AbrahamGGNT14,Filtser19,BLT07,BLT14} and \emph{translates} them to the distributed/parallel world.
Similar to the recent works of \cite{DBLP:conf/innovations/BeckerEL20} and  \cite{DBLP:conf/focs/RozhonEGH22}, we reduce the construction of a decomposition to a polylogarithmic number of approximate SSSP computations.

%All of our algorithms are heavily influenced by Weiman and Yurens' diameter approximation \cite{WeimanY13} and the machinery developed by Li and Parter to distributively compute the diameter of planar graphs \cite{DBLP:conf/stoc/LiP19}.
%Their core idea is to recursively remove separators from the graph and compute the shortest path trees for nodes on the separators.
%These trees can then be used to approximate all other paths.
%Further, these node can also be used to create clusters with low diameter and low overlap (by mixing ideas from \cite{DBLP:conf/stoc/AbrahamGGNT14}, \cite{Filtser19}, and \cite{BLT14}).
%We show that all these techniques also work with \emph{approximate distance} computations as we do how to compute exact distances in time $\Tilde{O}(\HD)$ in \CONGEST.
%The distances are instead computed by a recent breakthrough result by Rozhon \textcircled{r} Grunau \textcircled{r} Häupler \textcircled{r} Zuzic \textcircled{r} Li\footnote{Rozhon \textcircled{r} al. in the remainder.} \cite{DBLP:conf/stoc/RozhonGHZL22}.
%However, this prevents us Li and Parters' divide-and-conquer framework in a black-box fashion and we have to adapt certain parts of fit our needs.
%Instead, we add an extra partition step that \textbf{forces} the subgraphs that result from removing the separator (a) shrink in size, (b) maintain small (weighted) diameters, and (c) contain a constant fraction of all shortest paths between their nodes. 
%A careful analysis then reveals that these changes only add negligible error probability and a logarithmic blow-up of the runtime and the routing tables.  
%This step adds a small probability of error
%Interestingly, this new divide-and-conquer technique can also be applied to other sequential algorithms and allows for fast distributed implementation of a clustering algorithm of 
%Abraham, Gavoille, Gupta, Neiman and Talwar\cite{DBLP:conf/stoc/AbrahamGGNT14} and its improvement by Fitsler \cite{filtser}.


%For the routing scheme, we adapt the diameter approximations of Weimann and Yuster\cite{} and Li and Parter\cite{DBLP:conf/stoc/LiP19} that (with very little tuning) provide a routing scheme with additive stretch $\epsilon\cdot D$ where $D$ is the \emph{weighted} diameter. We combine these algorithms with low-diameter decompositions. We cluster the network into connected subgraphs of geometrically increasing diameter and apply the scheme on each subgraph, so for each pair of nodes there is a suitable path.
%The main technical challenge lies in the fast distributed implementation of this approach. 
%In particular, we must guarantee that the clusters are (almost) node-disjoint so the computations in each subgraph can be efficiently parallelized.
%
%
%We achieve this by (a) adding two additional partitioning steps to their algorithms, which ensure that it be efficiently parallelized und (b) replacing their exact distance computation with approximate ones that can be computed much faster than exact computations.
%For our other results, we develop a cluster algorithm inspired by an algorithms of Abraham, Gavoille, Gupta, Neiman and Talwar\cite{DBLP:conf/stoc/AbrahamGGNT14} and its improvement by Fitsler \cite{filtser}, and also mixes in ideas from Busch, LaFortune and Tirthapura \cite{BLT07,BLT14}.
%All these algorithms are sequential and we provide efficient distributed (and parallel) variants by combining it the divide-and-conquer framework we developed for our routing scheme.

%Finally, all of our scheme heavily rely on the Minor Aggregation Framework, which has received a lost of attention recently. 
%That is, our algorithms can be broken down to simple aggregation tasks on node disjoint subgraphs.





%In this work, we contribute further to this by presenting fast distributed algorithms for so-called \emph{compact} routing schemes for systems that can be modeled by weighted planar graphs. 
%Our techniques can further be used to construct sparse coverings, padded decompositions, and low diameter decompositions, which may be of independent interest.
%The goal of compact routing is to find routing schemes where (1) each device only has to store few information to execute the routing, and (2) the length of the resulting routing paths is within a constant factor of the best possible length.

%\paragraph{\textbf{Compact Routing}} To define compact routing, we will think of the distributed system as a weighted undirected graph $G := (V,E,w)$.
%The nodes $V$ model the devices of the distributed system and edges $E$ represent the connections between them.
%The weights denote the \emph{costs} for send a message along the edge.
%These weights could, for example, model the \emph{latency} between two nodes or the energy consumption for a wireless transmission, however, we do not restrict ourselves to any specific cost metric.
%Formally, we define a routing scheme $R$ for graph $G$ as a tuple $R := (\Lambda,P)$ where $\Lambda$ is a set of labels and $P$ is a set of local routing rules, which we call the routing tables.
%Each node $v \in V$ gets assigned a label $\lambda(v) \in \Lambda$ and a routing table $\rho_v: \Lambda \to V$.
%The label stores data that aids the routing scheme in finding a path, while
%the routing table is a function that maps every label to a neighbor of $v$ in $G$.
%Given a packet with the label $\lambda(t)$, any node must be able to forward this packet in the graph only using the label and its routing table such that it eventually reaches the intended %receiver. 
%More formally, for each pair $s,t \in V$ there is a path $P^R_{st} := (v_0 = s, \dots, v_\ell=t)$ with $v_{i+1} = \rho_{v_{i}}(\lambda(t))$.
%We measure the performance of a compact routing scheme $R$ by three factors \emph{preprocessing time}, \emph{stretch}, and \emph{label size}.
%The  Preprocessing Time $T_R$ is time it takes for a protocol compute all labels and routing tables. 
%This should be as small as possible, so the lables and tables can be quickly recomputed. 
%Further, the stretch $\alpha_R$ is the ratio between the length $d_R(s,t)$ of the path chosen by our routing scheme $R$ and the actual shortest path length $d_G(s,t)$ in the graph representing the network.
%More formally, it holds $\alpha_R := \max_{s,t \in V} \frac{d_R(s,t)}{d_G(s,t)}$.
%Obviously, we want the stretch to be as small as possible.
%Finally, the Label Size $\beta_R$ is the size of the biggest label $\lambda(v) \in \Lambda$, i.e., it holds $\beta_R := \max_{v \in V} |\lambda(v)|$.
%Note that a trivial label is simply a copy of the complete graph, which is obviously not a scalable solution as its size is $O(|E|)$.
%Instead we want the labels to contain few bits as possible because the label of the target is sent as part of every message.
%Unnecessarily big or bloated labels increase the message size and dampen the throughput.
%On a similar note, all nodes could simply store the full graph as their routing table, which also be infeasible.

%\paragraph{\textbf{Our Contribution}} 






%In the distributed version of the problem each node $v \in V$ has to compute a label $\lambda(v)$ and routing table $\rho(u)$ themselves by exchanging (small) messages with their neighbors.
%In this work, we present algorithm that computes a routing scheme with near-optimal path length that can efficiently computed.

%Finally, we say, a routing scheme is $(\alpha,\beta)$-competetive if it has stretch $\alpha$ and label size $\beta$.



==> Distributed Construction of Near-Optimal Compact Routing Schemes for Planar Graphs/Sections/Models.tex <==
\subsection{Model(s)}
In this work, we present a \emph{meta-algorithm} that can be implemented in several different models of computation for parallel and distributed systems. 
\todo{Mention Universally Optimal Algorithms}
In this section, we quickly introduce these models as well as a meta-model that will simplify the presentation of our results.
We begin with the two well-established models \CONGEST and the \PRAM, which are the de-facto standard models for distributed and parallel computing, respectively.
 
{\textbf{The \CONGEST model}}
We consider a graph $G = (V,E)$ that consists of $n$ nodes with unique identifiers.
Time proceeds in synchronous rounds.
In each round, nodes receive messages from the previous round;
they perform (unlimited) computation based on their internal states and the messages they have received so far; 
and finally, they send messages to their neighbors in $G$. 
The model will provide the most technical challenges and can be regarded as the \emph{main} model of this paper.

{\textbf{The $(\mathbf{CRCW}-)$\PRAM model}} 
The system consists of $p$ processors, each with a unique ID in $\{1, 2, \dots, p\}$, and a shared memory block of $M$ entries.
We assume that each processor is aware of its identifier.
Each processor can read from or write to \emph{any} memory entry in every round.
We assume \emph{concurrent reads}, i.e., multiple processors can simultaneously read the duplicate entry. Further, we assume \emph{concurrent writes}, i.e., an arbitrary value (out of the proposed values) is written if multiple processors write to the duplicate entry. The input graph $G$ is provided in the shared memory as an adjacency list, i.e., where there is a memory cell for the $j^{th}$ neighbor of the $i^{th}$ node that looks up in $O(1)$ time.

{\textbf{The \HYBRID model}} In addition to these two \emph{classic} models of computation, we will also use the recently established \HYBRID model. The \HYBRID model was introduced in \cite{AHKSS20} as a means to study distributed systems that leverage multiple communication modes of different characteristics, usually a \emph{local} and a \emph{global} mode. 
%Of particular interest are networks that combine a \emph{local} communication mode, which has a large bandwidth but is restricted to edges of a \emph{graph} on the nodes of the network, with a \emph{global} communication mode where any two nodes may communicate in principle, but very little such communication can take place per unit of time. 
%This concept captures various real distributed systems, notably networks of mobile computing devices that combine high bandwidth but locally restricted wireless communication on a \emph{unit-disc-graph} with data transmission via the cellular network.
%Note that algorithms for routing schemes in hybrid networks are of increasing importance, as contemporary communication standards support such settings, one prominent example being the 5G standard.
%The \HYBRID model restricts which nodes may communicate and to what extent. It combines local communication among nodes which requires little to no external infrastructure, for instance via ad-hoc networks among nodes that are physically close to each other, with overlay networks that utilize some shared infrastructure like a cellular network.
More precisely, the \emph{local} communication mode is modeled as a connected graph, in which each node is initially aware of its neighbors and is allowed to send a message of size $\lambda$ bits to each neighbor in each round. In the \emph{global} communication mode, each round, each node may send or receive $\gamma$ bits to/from every other node that can be addressed with its ID in $[n]$ in case it is known. If any restrictions are violated in a given round, an arbitrary subset of messages is dropped\footnote{Note that our algorithms never exploit this and ensure that no messages are dropped.}.
In this paper, we consider a weak form of the \HYBRID model, which sets $\lambda \in \bigO(\log n)$ and $\gamma \in \bigO(\log^2 n)$, which corresponds to the combination of the classic distributed models \CONGEST\footnote{Some previous papers that consider hybrid models use $\lambda = \infty$, i.e., the \LOCAL model as local mode.} as local mode, and $\mathsf{NODE \,\, CAPACITATED \,\, CLIQUE}$ 
(\NCC)\footnote{Our approach works for the stricter \NCCzero model where only incident nodes in the local network and those introduced can communicate globally.} presented in \cite{AGG+19} as global mode.
Note that this particular setup for this particular graph class can simulate all work-efficient \PRAM algorithms with logarithmic overhead.
This fact was shown in \cite{FHS20}:
\begin{lemma} \label{lem:spa:pram_sim}
    Let $G$ be a graph with arboricity\footnote{The arboricity is the number forests $G$ can be divided into or -equivalently - the maximum average degree of any subgraph.} $a$ and let $\mathcal{A}$ be a PRAM algorithm that solves a graph problem on $G$ using $N$ processors with depth $T$.
    A CRCW \PRAM algorithm $\mathcal{A}$ can be simulated in the \HYBRID mode with $\lambda \in \bigO(\log n)$ and $\gamma \in \bigO(\log^2 n)$ in  $O(a/(\log n) + T \cdot (N/n + \log n))=\Tilde{O}(T\cdot(\nicefrac{N}{n})+a)$ time, w.h.p.
\end{lemma}
The arboricity of the planar graph is $5$ \jinfeng{what is 5?}, and any \PRAM algorithm presented in this work can be simulated with logarithmic overhead.
We provide the details in Appendix \ref{appendix:pram_simulation}.
Note that, for all \HYBRID algorithms presented in this work, we will always use the simulation of the \PRAM algorithm.




==> Distributed Construction of Near-Optimal Compact Routing Schemes for Planar Graphs/Sections/Problem_Definition.tex <==
\subsection{Problem Definition}
Our goal is to compute routing schemes. To this end, we adapt the definition of \cite{X}\julian{cite elkin, neimann, thorup, zwick}:

\paragraph{\textbf{Routing Schemes}}
%Given a graph $G=(V,E)$, A \emph{routing scheme} consists of a \emph{labeling function} $\lambda: V\to \{0,1\}^\star$ that assigns a bit string to each node and a \emph{routing function} $\rho_v: \{0,1\}^\star \to V$\julian{alternative: one $\rho :V\times \{0,1\}^\star$} for each node $v\in V$ that maps a target nodes identifier to a neighboring node of $v$ the packet should be forwarded to. Additionally, for each pair of nodes $(s,t)$, the repeated evaluation of the routing functions yields a path $(v_0:=s, v_1:=\rho_s(\lambda(t),v_2:=\rho_{v_1}(\lambda(t),\dots, v_\ell:=t)$ from $s$ to $t$. We do not require these paths to be shortest. However, we rate the quality of a routing scheme by comparing the length of its paths with shortest paths. Specifically, a routing scheme has \emph{stretch} $\alpha$, if for every pair of nodes $(s,t)$, we have $\sum_{i=0}^{\ell-1} d(v_i,v_i+1) \leq \alpha\cdot d(s,t)$.
A routing scheme allows the nodes of a graph to forward messages towards a given target node by providing each node with some local information (a routing table) and a label assigning some information to a node that can be accessed to route packets towards it. This results in a natural separation of the problem into two phases: The preprocessing phase where routing tables and node labels are computed and the routing phase, where the nodes forward packages to their destinations. 
More specifically, in the routing phase, a packet that is to be routed is equipped with a header containing some routing information. 
Any node receiving this packet makes use of its routing table and the target label to decide which of its neighbors the packet should be forwarded to. For all of our algorithms, the header consists only of the target node's label.

The quality of a routing scheme can be measured with different quantities. We are specifically interested in (i) a routing scheme's stretch, i.e., the worst case ratio of the length of some routing path and the shortest path that could have been taken, (ii) its memory requirement, i.e., the size of its routing tables, the node labels and the amount of memory required to perform the preprocessing phase, and (iii) how efficient it can be computed, i.e., we are interested in the runtime of the preprocessing phase.
The latter two will heavily depend on the model of distributed computation that is assumed for the algorithm. As we will consider multiple models throughout the paper, we will also present multiple values for them.

%\begin{itemize}
%    \item allow nodes to forward packages using local information and header (target label)
%    \item local information: routing table
%    \item phases
%    \begin{itemize}
%        \item preprocessing phase: compute routing table and label
%        \item routing phase: forward packet using routing table and label (and header)
%    \end{itemize}
%    \item stretch: worst-case ratio of length of routing path and shortest path
%    \item compact tables and short labels
%    \item computation efficiency
%\end{itemize}

==> Distributed Construction of Near-Optimal Compact Routing Schemes for Planar Graphs/Sections/RelatedWork.tex <==
\paragraph{\textbf{Compact Routing}} The is a vast amount of research on compact routing schemes for general graphs and specific graph classes.
In most of these works, the focus lies on achieving the best possible stretch with the lowest possible memory.
As mentioned in the introduction, the preprocessing time takes a backseat.
For general graphs, Thorup and Zwick described a scheme with stretch $2k-1$ that creates labels of size $O(k\log n)$ and routing tables of size $O(n^{\frac{1}{k}})$ which is essentially tight.
This groundbreaking work was followed by a plethora of optimal compact routing schemes for specific graph classes and metrics. 
Among these are minor-free graphs (which include planar graphs), graphs of bounded doubling dimension, and graphs embedded in a euclidean plane, 
just to name a few. 
\thorsten{Maybe there is a survey? }


\paragraph{\textbf{Fast Distributed Routing Tables}} 
Like in our work, they rely on sparse \emph{covering} to build their routing.
However, they construct them in a completely different way.
Further, note that solving the APSP problem solves the routing scheme problem.
Here, the currently fasted algorithms require $O(n^{\frac{5}{4}})$ (randomized) and $O(n^{\frac{3}{2}})$ (deterministic).

\paragraph{\textbf{Shortest Paths and Routing Schemes in Hybrid Networks.}} Previous work in the \HYBRID model has mostly focused on shortest path problems \cite{Augustine2020, Kuhn2020, Feldmann2020, CensorHillel2021, Anagnostides2021}. 
Here, neither the lower bound of \CONGEST nor \LOCAL hold, so one can hope for $o(\HD)$ time algorithms.
The complexity of APSP is essentially settled: \cite{Augustine2020, Kuhn2020} give an algorithm taking $\tilO(\!\sqrt{n})$ rounds (where $\tilO$ hides $\polylog n$ factors), which is tight.
%The state-of-the-art algorithm for exact SSSP is provided by \cite{CensorHillel2021} and takes $\bigO(n^{1/3})$ rounds.$^{\ref{ftn:powerful_hybrid}}$ A recent result implies that a $(1\p\eps)$ approximation of SSSP is possible in $\tilO(1)$ rounds even with the weaker combination of \CONGEST and \NCC which we consider in this work. This is due to \cite{Zuzic2022} which solves SSSP by $\tilO(1)$ applications of ``part-wise aggregation'' on the network. An \textit{exact, deterministic} solution for SSSP in $\bigO(\log n)$ rounds has been achieved on specific classes of graphs (e.g.~cactus graphs, which includes trees) by \cite{Feldmann2020}. Another exact SSSP algorithm that takes $\tilO(\!\sqrt{SPD})$ rounds (where $SPD$ is the shortest-path-diameter of the local graph) is provided by \cite{Augustine2020}.
In a recent article, \cite{Kuhn2022} considers computing routing schemes in the \HYBRID model on general graphs: they show that in $\tilO(n^{1/3})$ rounds one can compute \textbf{exact} routing schemes with labels of size $\tilO(n^{2/3})$ bits, or constant stretch approximations with smaller labels of $\bigO(\log n)$ bits. Interestingly, \cite{Kuhn2022} also gives lower bounds: they show that it takes $\tilOm(n^{1/3})$ rounds to compute exact routing schemes that hold for relabeling of size $\bigO(n^{2/3})$ and on unweighted graphs. They also give polynomial lower bounds for constant approximations on weighted graphs, implying that to overcome this lower bound in round complexity and label size, the restriction to a class of graphs is necessary!
Further, some works do this and consider $(O(1),\widetilde{O}(1))$-competitive routing schemes for UDGs, i.e., ad-hoc sensor networks.
First, there is a paper by Castenow, Kolb, and Scheideler which presents a $O(1)$-competitive routing scheme that requires $O(h)$ time and space where $h$ is the number of radio holes in the UDG, i.e., the number of connected areas with no coverage enclosed by the nodes. However, they require that the bounding boxes of two radio holes do not overlap and nodes within a bounding box do not get a label. 
Second, there is a work by Coy et al. \cite{Coy2022}, in which they show how to compute a routing scheme for a UDG without holes in $O(\log(n))$ time and space by computing a routing scheme for a corresponding grid graph.
In a recent extension, an algorithm that also supports radio holes is presented. It requires $O(h^2+\log(n))$ time and is -- in stark contrast to our algorithm -- completely deterministic.







==> Sections/Dump/ClusteringToCovering.tex <==
Now suppose  that we have black-boc access to a padded decomposition algorithm \textsc{Decomp}(d) that runs in time $T_{DC}$.
This provides us a straightforward construction of a $(e^{\frac{\tau}{k}}\log^2(n),O(k))$-nice clustering in $O(e^{\frac{\tau}{k}}\log^2(n))$
given that graph's diameter is polynomial in $n$.
To this end, let $D \in O(n^c)$ be the graph's diameter and define $\Delta_i = 2^i$ for every $i=1, \dots, \log(D)$.
Note that our assumption ensures that it holds $i < c\log(n)$ and therefore $i$ is logarithmic in $n$.

\begin{algo}
\textbf{\underline{\texttt{CreateNiceClustering}}}($G$)
\begin{enumerate}
    \item Let $\mathfrak{C} = \emptyset$ be an empty clustering.
    \item For each $i \in [1,\log(D)]$ do the following:
    \begin{enumerate}
        \item Create $\tau_k$ padded decompositions with distance parameter $\Delta_i$. 
        \item Denote the resulting decompositions as $\mathcal{C}^i := \{C^{(i)}_1, \dots, C^{(i)}_{\tau_k}\}$, s.t., it holds:
        \begin{align}
            C^{(i)} := \textsc{Decomp}(G,\Delta_i)
        \end{align}
        \item Add all clusters from $\mathcal{C}^i$ to $\mathfrak{C}$.
    \end{enumerate}
    \item Return $\mathfrak{C}$  
\end{enumerate}    
\end{algo}

Since each $v$ is in exactly one cluster per decomposition, the total number of clusters that contain $v$ is $\alpha\log(n)\log(D)$.
Further, for any pair of nodes $s,t \in V$ with distance $d(s,t)$ there is cluster with a diameter $O(d(s,t))$ that contains both $s$ and $t$.
Then, we can use the center of this cluster as a \emph{routing beacon} for $s$ and $t$.

By that, we mean that our routing scheme picks a path $P_{svt} := (s \to v \to t)$ approximates the path $P_{st} = (s \to t)$.

==> Sections/Dump/OldProof.tex <==
\begin{appendixproof}

Let us introduce some more notation and properties before proving this Lemma.
Define the following events:
\begin{alignat*}{2}
\calC_i &= \{B_z\cap K_i\notin\{\emptyset,B_z\}\} & \qquad &
\text{``$B_z$ cut in round $i$ (by $A_i$)''}, \\
\calF_i &= \{B_z\cap K_i=\emptyset\} & & \text{``$i$ was a \texttt{no-op}
  round''}, \\
\calE_i &= \bigg\{\calC_i\wedge\bigwedge_{j<i}\calF_j\bigg\} & &
\text{``$B_z$ first cut in round $i$''.}
\end{alignat*}

Denote by $\calF_{(< i)}$ the event $\bigwedge_{j<i}\calF_j$, so that $\calE_i =
(\calC_i \land \calF_{(<i)})$.
Denote by $\calFbar_i$ the complement of $\calF_i$. Observe that $\calC_i$ (respectively $\calFbar_i$) implies that $A_i\in\calI_z$, so
\begin{eqnarray}\label{eq:full1}
\Pr[\calC_i]=\Pr[\calC_i\wedge A_i\in\calI_z]=\Pr[A_i\in\calI_z]\cdot\Pr[\calC_i\mid A_i\in\calI_z]~,\\\label{eq:full2}
\Pr[\calFbar_i]=\Pr[A_i\in\calI_z]\cdot\Pr[\calFbar_i\mid A_i\in\calI_z]~.
\end{eqnarray}
and the same holds also when conditioning on any other event. We have the following claim:

\begin{claim}\label{claim:cut}
For each $i\in N$,
\[
\Pr[\calC_i\mid \calF_{(<i)}, A_i\in\calI_z]\le (1-\delta)\cdot\left(\Pr[\calFbar_i\mid \calF_{(<i)},A_i\in \calI_z]+\frac{1}{e^b-1}\right)~.
\]
\end{claim}
\begin{proof}
Fix any graph $G_i$ and any set $A_i\subseteq V(G_i)$ that agree with the conditioning on $\calF_0,\dots \calF_{i-1}$ and so that $A_i\in \calI_z$. Denote by $\rho=d_{G_i}(A_i,B_z)$, $\bar{b}=b/(u-l)$, and let $m=\max\{l,\rho\}$ . Recall that $R_i$ is chosen independently, so
\begin{eqnarray*}
\Pr[\calFbar_i\mid \calF_0,\dots,\calF_{i-1},A_i\in \calI_z,A_i]&=&\int_m^u\frac{\bar{b} e^{-\bar{b}y}}{e^{-\bar{b}l}-e^{-\bar{b}u}}dy\\
&=&\frac{e^{-\bar{b}m}-e^{-\bar{b}u}}{e^{-\bar{b}l}-e^{-\bar{b}u}}~.
\end{eqnarray*}
Since $\calF_0,\dots,\calF_{i-1}$ occurred and $G_i\supseteq G_0\setminus(\cup_{j<i}K_j)$, we have that $B_z\subseteq
G_i$. Now if $R_i\ge\rho+2\gamma$ then by the triangle inequality
$B_z\subseteq K_i$, and the ball is ``saved''. This bounds the cut
probability thus:
\begin{eqnarray*}
\Pr[\calC_i\mid \calF_{(<i)},A_i\in \calI_z,A_i]&\le&\int_m^{\rho+2\gamma}\frac{\bar{b} e^{-\bar{b}y}}{e^{-\bar{b}l}-e^{-\bar{b}u}}dy\\
&\le&\frac{e^{-\bar{b}m}-e^{-\bar{b}(m+2\gamma)}}{e^{-\bar{b}l}-e^{-\bar{b}u}}\\
&=&\frac{e^{-\bar{b}m}(1-\delta)}{e^{-\bar{b}l}-e^{-\bar{b}u}}\\
&=&(1-\delta)\cdot\Pr[\calFbar_i\mid \calF_{(<i)},A_i\in \calI_z,A_i]+(1-\delta)\frac{e^{-\bar{b}u}}{e^{-\bar{b}l}-e^{-\bar{b}u}}\\
&=& (1-\delta)\cdot\left(\Pr[\calFbar_i\mid \calF_{(<i)},A_i\in \calI_z,A_i]+\frac{1}{e^b-1}\right)~.
\end{eqnarray*}
Finally, because the bound holds for any $A_i$, it holds without
conditioning on it.
\end{proof}


\begin{proof}[Proof of \ref{lem:cut}]

Observe that for each $i\in[N]$, the events $\left\{\calFbar_i\wedge\calF_{(<i)}\right\}$ are pairwise disjoint (this is the event that $B_z$ is either cut or contained in $K_i$ for the first time),
thus by the law of total probability,
\begin{equation}\label{eq:gq}
\sum_{i\in N}\Pr\left[\calFbar_i\wedge\calF_{(<i)}\right]\le 1~.
\end{equation}
Also, by the linearity of expectation
\begin{equation}\label{eq:lin}
\tau = \sum_{i \in }\Pr[A_i\in\calI_z]~.
\end{equation}
To bound the probability of the ball being cut, we start off with the
trivial union bound:
\begin{align*}
\Pr\left[\bigcup_{i\in N}\calE_i\right]&\le \sum_i\Pr[\calE_i] = \sum_i\Pr\left[\calC_i\wedge\calF_{(<i)}\right]\\
&=\sum_i\Pr[\calC_i\mid \calF_{(<i)}] \cdot \Pr[\calF_{(<i)}] \\
&\stackrel{\eqref{eq:full1}}{=}
  \sum_i \Pr[\calC_i \mid \calF_{(<i)}, A_i\in\calI_z]
  \cdot \Pr[A_i\in\calI_z\mid \calF_{(<i)}]
  \cdot \Pr[\calF_{(<i)}] \\
&\stackrel{\text{\footnotesize \ref{claim:cut}}}{\leq}
  \sum_i (1-\delta)\left(\Pr[\calFbar_i\mid \calF_{(<i)},A_i\in\calI_z]+\frac{1}{e^b-1}\right)
  \cdot \Pr[A_i\in\calI_z\mid \calF_{(<i)}]
  \cdot \Pr[\calF_{(<i)}] \\
 &\stackrel{\eqref{eq:full2}}{=} (1-\delta)\cdot\sum_i\Pr\left[\calFbar_i\wedge\calF_{(<i)}\right]+\sum_i\Pr\left[A_i\in\calI_z\wedge\calF_{(<i)}\right]\cdot\frac{1-\delta}{e^b-1}\\
 &\stackrel{\eqref{eq:gq}}{\le}(1-\delta)+\frac{1-\delta}{e^b-1}\cdot\sum_i\Pr[A_i\in\calI_z]\\
 &\stackrel{\eqref{eq:lin}}{=}(1-\delta)\left(1+\frac{\tau}{e^b-1}\right)~.
\end{align*}
This completes the proof.
\end{proof}

\end{appendixproof}

==> Sections/Problem_Definition.tex <==
\subsection{Problem Definition}
Our goal is to compute routing schemes. To this end, we adapt the definition of \cite{X}\julian{cite elkin, neimann, thorup, zwick}:

\paragraph{\textbf{Routing Schemes}}
%Given a graph $G=(V,E)$, A \emph{routing scheme} consists of a \emph{labeling function} $\lambda: V\to \{0,1\}^\star$ that assigns a bit string to each node and a \emph{routing function} $\rho_v: \{0,1\}^\star \to V$\julian{alternative: one $\rho :V\times \{0,1\}^\star$} for each node $v\in V$ that maps a target nodes identifier to a neighboring node of $v$ the packet should be forwarded to. Additionally, for each pair of nodes $(s,t)$, the repeated evaluation of the routing functions yields a path $(v_0:=s, v_1:=\rho_s(\lambda(t),v_2:=\rho_{v_1}(\lambda(t),\dots, v_\ell:=t)$ from $s$ to $t$. We do not require these paths to be shortest. However, we rate the quality of a routing scheme by comparing the length of its paths with shortest paths. Specifically, a routing scheme has \emph{stretch} $\alpha$, if for every pair of nodes $(s,t)$, we have $\sum_{i=0}^{\ell-1} d(v_i,v_i+1) \leq \alpha\cdot d(s,t)$.
A routing scheme allows the nodes of a graph to forward messages towards a given target node by providing each node with some local information (a routing table) and a label assigning some information to a node that can be accessed to route packets towards it. This results in a natural separation of the problem into two phases: The preprocessing phase where routing tables and node labels are computed and the routing phase, where the nodes forward packages to their destinations. 
More specifically, in the routing phase, a packet that is to be routed is equipped with a header containing some routing information. 
Any node receiving this packet makes use of its routing table and the target label to decide which of its neighbors the packet should be forwarded to. For all of our algorithms, the header consists only of the target node's label.

The quality of a routing scheme can be measured with different quantities. We are specifically interested in (i) a routing scheme's stretch, i.e., the worst case ratio of the length of some routing path and the shortest path that could have been taken, (ii) its memory requirement, i.e., the size of its routing tables, the node labels and the amount of memory required to perform the preprocessing phase, and (iii) how efficient it can be computed, i.e., we are interested in the runtime of the preprocessing phase.
The latter two will heavily depend on the model of distributed computation that is assumed for the algorithm. As we will consider multiple models throughout the paper, we will also present multiple values for them.

%\begin{itemize}
%    \item allow nodes to forward packages using local information and header (target label)
%    \item local information: routing table
%    \item phases
%    \begin{itemize}
%        \item preprocessing phase: compute routing table and label
%        \item routing phase: forward packet using routing table and label (and header)
%    \end{itemize}
%    \item stretch: worst-case ratio of length of routing path and shortest path
%    \item compact tables and short labels
%    \item computation efficiency
%\end{itemize}

==> Sections/RelatedWork.tex <==
\paragraph{\textbf{Compact Routing}} The is a vast amount of research on compact routing schemes for general graphs and specific graph classes.
In most of these works, the focus lies on achieving the best possible stretch with the lowest possible memory.
As mentioned in the introduction, the preprocessing time takes a backseat.
For general graphs, Thorup and Zwick described a scheme with stretch $2k-1$ that creates labels of size $O(k\log n)$ and routing tables of size $O(n^{\frac{1}{k}})$ which is essentially tight.
This groundbreaking work was followed by a plethora of optimal compact routing schemes for specific graph classes and metrics. 
Among these are minor-free graphs (which include planar graphs), graphs of bounded doubling dimension, and graphs embedded in a euclidean plane, 
just to name a few. 
\thorsten{Maybe there is a survey? }


\paragraph{\textbf{Fast Distributed Routing Tables}} 
Like in our work, they rely on sparse \emph{covering} to build their routing.
However, they construct them in a completely different way.
Further, note that solving the APSP problem solves the routing scheme problem.
Here, the currently fasted algorithms require $O(n^{\frac{5}{4}})$ (randomized) and $O(n^{\frac{3}{2}})$ (deterministic).

\paragraph{\textbf{Shortest Paths and Routing Schemes in Hybrid Networks.}} Previous work in the \HYBRID model has mostly focused on shortest path problems \cite{Augustine2020, Kuhn2020, Feldmann2020, CensorHillel2021, Anagnostides2021}. 
Here, neither the lower bound of \CONGEST nor \LOCAL hold, so one can hope for $o(\HD)$ time algorithms.
The complexity of APSP is essentially settled: \cite{Augustine2020, Kuhn2020} give an algorithm taking $\tilO(\!\sqrt{n})$ rounds (where $\tilO$ hides $\polylog n$ factors), which is tight.
%The state-of-the-art algorithm for exact SSSP is provided by \cite{CensorHillel2021} and takes $\bigO(n^{1/3})$ rounds.$^{\ref{ftn:powerful_hybrid}}$ A recent result implies that a $(1\p\eps)$ approximation of SSSP is possible in $\tilO(1)$ rounds even with the weaker combination of \CONGEST and \NCC which we consider in this work. This is due to \cite{Zuzic2022} which solves SSSP by $\tilO(1)$ applications of ``part-wise aggregation'' on the network. An \textit{exact, deterministic} solution for SSSP in $\bigO(\log n)$ rounds has been achieved on specific classes of graphs (e.g.~cactus graphs, which includes trees) by \cite{Feldmann2020}. Another exact SSSP algorithm that takes $\tilO(\!\sqrt{SPD})$ rounds (where $SPD$ is the shortest-path-diameter of the local graph) is provided by \cite{Augustine2020}.
In a recent article, \cite{Kuhn2022} considers computing routing schemes in the \HYBRID model on general graphs: they show that in $\tilO(n^{1/3})$ rounds one can compute \textbf{exact} routing schemes with labels of size $\tilO(n^{2/3})$ bits, or constant stretch approximations with smaller labels of $\bigO(\log n)$ bits. Interestingly, \cite{Kuhn2022} also gives lower bounds: they show that it takes $\tilOm(n^{1/3})$ rounds to compute exact routing schemes that hold for relabeling of size $\bigO(n^{2/3})$ and on unweighted graphs. They also give polynomial lower bounds for constant approximations on weighted graphs, implying that to overcome this lower bound in round complexity and label size, the restriction to a class of graphs is necessary!
Further, some works do this and consider $(O(1),\widetilde{O}(1))$-competitive routing schemes for UDGs, i.e., ad-hoc sensor networks.
First, there is a paper by Castenow, Kolb, and Scheideler which presents a $O(1)$-competitive routing scheme that requires $O(h)$ time and space where $h$ is the number of radio holes in the UDG, i.e., the number of connected areas with no coverage enclosed by the nodes. However, they require that the bounding boxes of two radio holes do not overlap and nodes within a bounding box do not get a label. 
Second, there is a work by Coy et al. \cite{Coy2022}, in which they show how to compute a routing scheme for a UDG without holes in $O(\log(n))$ time and space by computing a routing scheme for a corresponding grid graph.
In a recent extension, an algorithm that also supports radio holes is presented. It requires $O(h^2+\log(n))$ time and is -- in stark contrast to our algorithm -- completely deterministic.






